GASLITEing the Retrieval: Exploring Vulnerabilities in Dense Embedding-based Search

Dense embedding-based text retrieval$\unicode{x2013}$retrieval of relevant passages from corpora via deep learning encodings$\unicode{x2013}$has emerged as a powerful method attaining state-of-the-art search results and popularizing Retrieval Augmented Generation (RAG). Still, like other search methods, embedding-based retrieval may be susceptible to search-engine optimization (SEO) attacks, where adversaries promote malicious content by introducing adversarial passages to corpora. Prior work has shown such SEO is feasible, mostly demonstrating attacks against retrieval-integrated systems (e.g., RAG). Yet, these consider relaxed SEO threat models (e.g., targeting single queries), use baseline attack methods, and provide small-scale retrieval evaluation, thus obscuring our comprehensive understanding of retrievers' worst-case behavior. This work aims to faithfully and thoroughly assess retrievers' robustness, paving a path to uncover factors related to their susceptibility to SEO. To this end, we, first, propose the GASLITE attack for generating adversarial passages, that$\unicode{x2013}$without relying on the corpus content or modifying the model$\unicode{x2013}$carry adversary-chosen information while achieving high retrieval ranking, consistently outperforming prior approaches. Second, using GASLITE, we extensively evaluate retrievers' robustness, testing nine advanced models under varied threat models, while focusing on pertinent adversaries targeting queries on a specific concept (e.g., a public figure). Amongst our findings: retrievers are highly vulnerable to SEO against concept-specific queries, even under negligible poisoning rates (e.g., $\geq$0.0001% of the corpus), while generalizing across different corpora and query distributions; single-query SEO is completely solved by GASLITE; adaptive attacks demonstrate bypassing common defenses; [...]

==> more-macros.tex <==
\makeatletter
\newcommand\ctextBorder[1][blue]{%
  \UseName{str_if_eq:nnF}{#1}{blue}{\colorlet{ul}{#1}}%
  \ctextBorder@}

\ulposdef\ctextBorder@[xoffset-start=2pt]{%
    \ifulstarttype{0}%
        {\tcbset{ULsiderule/.append style={leftrule=1pt}}}%
        {\tcbset{ULsiderule/.append style={leftrule=0pt,sharp corners=west}}}%
    \ifulendtype{0}%
        {\tcbset{ULsiderule/.append style={rightrule=1pt,right=-0.5pt}}}%
        {\tcbset{ULsiderule/.append style={rightrule=0pt,sharp corners=east,right=-2pt}}}%
    \mybox[ULsiderule]{\vphantom{Ap}\rule{\ulwidth}{0pt}}%
  }
\makeatother



